User Information Augmented Semantic Frame Parsing using Coarse-to-Fine Neural Networks

Semantic frame parsing is a crucial component in spoken language understanding (SLU) to build spoken dialog systems. It has two main tasks: intent detection and slot filling. Although state-of-the-art approaches showed good results, they require large annotated training data and long training time. In this paper, we aim to alleviate these drawbacks for semantic frame parsing by utilizing the ubiquitous user information. We design a novel coarse-to-fine deep neural network model to incorporate prior knowledge of user information intermediately to better and quickly train a semantic frame parser. Due to the lack of benchmark dataset with real user information, we synthesize the simplest type of user information (location and time) on ATIS benchmark data. The results show that our approach leverages such simple user information to outperform state-of-the-art approaches by 0.25% for intent detection and 0.31% for slot filling using standard training data. When using smaller training data, the performance improvement on intent detection and slot filling reaches up to 1.35% and 1.20% respectively. We also show that our approach can achieve similar performance as state-of-the-art approaches by using less than 80% annotated training data. Moreover, the training time to achieve the similar performance is also reduced by over 60%.

==> body/old/approach_enc_dec.tex <==
\section{Proposed Approaches}\label{sc:approach}

In this section, we design our approaches based on the state-of-the-art model for intent detection and slot filling \cite{liu2016attention}.
We first describe the network structure, called progressive neural networks model, followed by a detailed training algorithm.

\subsection{Progressive Neural Networks Models}


As the name indicates, our main idea is to train the semantic frame parsing model progressively with an intermediate task before achieving the final goal of intent detection and slot filling.
This is motivated by the recent success of progressive neural networks \cite{Rusu2016progressive}.
Specifically, for each utterance $\vec{x}$, we first define the user context sequence $\vec{z}$ using the user context tree described in \kproblem problem definition.
Table \ref{table:atis_example_context} shows an example from ATIS dataset.
To this end, our approaches first train the context tagging model to derive $\vec{z}$ and then distill user context information based their corresponding semantic meanings to continue training the semantic frame parsing. 


\setlength{\tabcolsep}{0.5em}
\begin{table}[h]\scriptsize
	\centering
	\caption{ATIS corpus sample with context sequence (in gray)}
	\label{table:atis_example_context}
	\begin{tabular}{c|c|c|c|c|c|c}
		\toprule
		\textbf{utterance} ($\vec{x}$) & list & flights & between & la & and & boston \\
		\midrule
		\rowcolor{Gray}
		\textbf{context seq} ($\vec{z}$) &  O & O & O & B-Loc & O & B-Loc \\
		\midrule
		\textbf{slots} ($\vec{y}$) & O & O & O & B-FromLoc & O & B-ToLoc \\
		\bottomrule		
	\end{tabular}
\end{table}

Next, we first present our proposed models with only B- and O- format for the sake of clear presentation.
We then discuss the progressive training algorithm and how IOB format is supported in our models.

\subsubsection{Progressive RNN Encoder-Decoder Model}


Figure \ref{fig:rnn_enc_dec} shows the progressive RNN encoder-decoder model.
It consists of four main components as follows.


\begin{figure}[t]
	\centering
	\includegraphics[width=1\columnwidth,height=60mm]{rnn_enc_dec}
	\caption{Progressive RNN Encoder-Decoder Model}
	\label{fig:rnn_enc_dec}
\end{figure}

\vspace{2pt}
\noindent\textbf{Utterance Encoder:}
We use the same bidirectional RNN encoder with LSTM cells (BiLSTM) as in \cite{liu2016attention}.
The encoder hidden state $\vec{h}_t$ at each time step $t$ is the concatenation of forward state $\vec{fh}_t$ and backward state $\vec{bh}_t$, i.e., $\vec{h}_t = \vec{fh}_t \oplus \vec{bh}_t$.
The final hidden state $\vec{h}_T$, considered as hidden state of encoder $\vec{h}_e$, is used for all decoders as their initial state.




\vspace{2pt}
\noindent\textbf{Context Tagging Decoder:}
The context tagging decoder labels the context type for each word in the input utterance, which uses a unidirectional RNN with LSTM as its basic cell.
Since the labeling is based on the language context of input utterance, we follow the previous work \cite{liu2016attention} to use a language context vector $\vec{c}$ via the weighted sum of encoder states in which each $c_t = \sum_{k=1}^T \alpha_{t,k} h_k$ where $\vec{h}=(h_1,\ldots,h_T)$ and $\alpha_{t,j} = \textsl{softmax}(e_{i,j})$.
$e_{t,k}$ is also learned from a feed forward neural network $g$.
At each time step $t$, the LSTM state $s_t^c$ of context tagging decoder is computed as $s_t^c = f_\textsf{LSTM} (s_{t-1}^c, h_{t-1} \oplus c_{t-1})$ where $s_{t-1}^c$ is the state in previous time step and the concatenation of $h_{t-1}$ and $c_{t-1}$, i.e., $h_{t-1} \oplus c_{t-1}$, is used as the input for LSTM cell.
At last, we calculate the softmax output $P_t(z)$ for each word $i$ and use it to predict its context tag $\tilde{z}_t$:
\begin{equation}
P_c(t) = \textsl{softmax} (\matrix{W}_c s_t^c);\;\; \tilde{z}_t = \arg\max_{\theta_c} P_c(t)
\end{equation}



\vspace{2pt}
\noindent\textbf{Slot Filling Decoder:}
This is the key for distilling user context information into the model to help reduce the need of annotated training data.
It shares the same hidden state $h_t$ and language context $c_t$ with context tagging decoder.
We next discuss how to distill the external knowledge from user context information and combine all of them together.


For the tagged words related to each type of user context, we use external knowledge to derive the context distance vector $\vec{d}_t$ for each time stamp $t$, i.e., $\vec{d}_t = (d_t^1, \ldots, d_t^m)$ where $m$ is the number of user context types.
To this end, each element $d_t^j$ in context distance vector $\vec{d}_t $ is defined as follows:
\begin{equation}
d_t^j = \textsl{sigmoid} (\alpha_j \odot \textsl{dist}_t^j ) 
\end{equation}
where $\alpha_j$ is a trainable vector.

Next, we define the calculation of distance $\textsl{dist}_t^j$ for context $j$, through the example in Figure \ref{fig:rnn_enc_dec}.
\textit{W.l.o.g.}, we assume distances $d_t^1$ and $d_t^2$ correspond to two types of context, location and time, respectively.
Taking the second word \textsl{``LA"} as an example, we have its following location context distance since it is tagged as \textsl{``Location"} context:
$$\textsl{dist}_\textsl{loc}\textsl{(``LA", ``Pasadena")} \approx \textsl{10.7 (miles)}$$ by using external location based services, i.e., Google geocoding.
As \textsl{``LA"} is not relevant to time context, we set its time context distance: $$\textsl{dist}_\textsl{time}\textsl{(``LA", ``03/01/1993")} = -1$$


To feed the context vector $\vec{d}_t$ into the slot filling decoder, we weight the each element $d_t^j$ and the language context $c_t$ over the softmax probability distribution $P(z_t)$ from context tagging decoder.
Intuitively, this determines how important a user context information or the language context in utterance is to predict the slot tag of each word in the utterance.
Thus, we have the input $\Phi_t$ of LSTM cell at each time step $i$ in slot filling decoder as follows:
\begin{equation}
\Phi_t = P_c^1(t) d_t^1 \oplus \ldots \oplus P_c^m(t) d_t^m \oplus P_o(t) c_t
\end{equation}
where $P_c^j(z_t)$ and $P_o(z_t)$ stand for the probability that the $i^\textsl{th}$ word is predicted as context tag $j$ and not a context tag.
\emph{Note that we will discuss how to deal with IOB format in Section \ref{sc:approach:iob}.}
At last, similar as context tagging decoder, the LSTM state $s_t^s$ at time step $t$ is computed as $s_t^s = f_\textsf{LSTM} (s_{t-1}^s, h_{t-1} \oplus \Phi_{t-1})$ where $s_{t-1}^s$ is the state in previous time step.
And the slot tag is predicted as follows:
\begin{equation}
P_s(t) = \matrix{W}_s s_t^s;\;\; \tilde{y}_t = \arg\max_{\theta_s} P_s(t)
\end{equation}


\vspace{2pt}
\noindent\textbf{Intent Detection Decoder:}
We add an additional intent detection decoder as in \cite{liu2016attention} to generate the probability distribution $P_I$ of intent class labels from encoder hidden state $\vec{h}_e$.
\begin{equation}
P_I(\vec{x}) = P_I(\vec{h}_e) = \matrix{W}_I \vec{h}_e;\;\; \tilde{I} = \arg\max_{\theta_I} P_I(\vec{x})
\end{equation}


\noindent\textbf{\em Remarks:}
The sharing of hidden state $\vec{h}_i$ and language context $\vec{c}_i$ between context tagging and slot filling decoder is crucial to leverage the user context information.
For context tagging decoder, $\vec{h}_i, \vec{c}_i$ is mainly used to tag the words which belong to one type of user contexts.
The semantic slots of these words can be easily tagged in slot filling decoder by utilizing the distilled knowledge from user context instead of using $\vec{h}_i, \vec{c}_i$ again.
The slot filling then depends on $\vec{h}_i, \vec{c}_i$ to tag the other non-user-context words that are tagged ``O" in context tagging.



\subsubsection{Progressive Attention-based RNN Model}

\todo{...}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\columnwidth,height=60mm]{attention_rnn}
	\caption{Progressive Attention based RNN Model}
	\label{fig:attention_rnn}
\end{figure}





\subsection{Progressive Training with IOB Format Support}\label{sc:approach:training}


\subsubsection{Training Algorithm}

The training is conducted progressively step by step.
The first step is to train context tagging model with loss $\mathcal{L}_c$ as follows:
\begin{equation}
\mathcal{L}_c (\theta_e, \theta_c) \triangleq - {1 \over 2|C|+1} \sum_{i=1}^{2|C|+1} \sum_{t=1}^n z_t^i \log P_c^i(t)
\end{equation}
where $|C|$ is the number of context types.
The number $2|C| + 1$ comes from the I- and B- format for each type with O- format.

Then, we fix the parameters $\theta_c$ in context tagging decoder/RNN and train the slot filling decoder/RNN with loss $\mathcal{L}_c$ and intent classifier with loss $\mathcal{L}_I$ simultaneously.
\begin{equation}
\mathcal{L}_s (\theta_e, \theta_I, \theta_s) \triangleq - {1 \over 2|S|+1} \sum_{i=1}^{2|S|+1} \sum_{t=1}^n y_t^i \log P_s^i(t)
\end{equation}

\begin{equation}
\mathcal{L}_I (\theta_e, \theta_I, \theta_s) \triangleq - {1 \over |I|} \sum_{i=1}^{|I|} I^i_\vec{x} \log P_I^i(\vec{x})
\end{equation}
where $|S|$ and $|I|$ are the number of slots and intents.
$P^i$ stands for the probability $P(X=x_i)$.
Moreover, $\theta_e, \theta_c, \theta_s, \theta_I$ are the parameters in utterance, context tagging, slot filling and intent detection components in our proposed model.


\subsubsection{IOB Format Support}\label{sc:approach:iob}


Thanks to the progressive training procedure, the IOB format will be naturally supported in our models.
As in Figure \ref{fig:iob}, in the case of \textsl{``Los Angeles"} with ``B-Loc I-Loc", we take them together to extract the distance $\textsl{dist}_\textsl{loc}\textsl{(``Los Angeles", ``Pasadena")}$ from external resources.
Moreover, since B-Loc and I-Loc are considered as different tags in the output $P_c(t)$ of context tagging component, it can be directly used to infer B-FromLoc and I-FromLoc in slot filling component accordingly with distilled user context.

In the case that the type of context for the $i^\textsl{th}$ word is incorrectly tagged, the hidden state $\vec{h}_i$ and language context $\vec{c}_i$ will be used to infer the slot tags since the context tagging component output $P_c(t)$ will weight more on $\vec{h}_i, \vec{c}_i$ in this case.



\begin{figure}[h]
	\centering
	\includegraphics[width=0.9\columnwidth]{iob_distillation}
	\caption{Context Distillation in IOB Format}
	\label{fig:iob}
\end{figure}


==> body/simple_approach.tex <==
\section{Proposed First-Cut Approaches}

==> template/IS2018_paper_kit/LaTeX/IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************


